Optimizing Collision Avoidance in Dense Airspace using Deep Reinforcement Learning

New methodologies will be needed to ensure the airspace remains safe and efficient as traffic densities rise to accommodate new unmanned operations. This paper explores how unmanned free-flight traffic may operate in dense airspace. We develop and analyze autonomous collision avoidance systems for aircraft operating in dense airspace where traditional collision avoidance systems fail. We propose a metric for quantifying the decision burden on a collision avoidance system as well as a metric for measuring the impact of the collision avoidance system on airspace. We use deep reinforcement learning to compute corrections for an existing collision avoidance approach to account for dense airspace. The results show that a corrected collision avoidance system can operate more efficiently than traditional methods in dense airspace while maintaining high levels of safety.

==> atms2019_li/pics/encounter.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[]
        \node[] (encounter) at (0,0) {\includegraphics[scale=0.5]{atms2019_li/pics/encounter.pdf}};
        \node[aircraft top,fill=black,minimum width=1.3cm] (ownship) at (0,-0.06) {};
    \end{tikzpicture}
    \caption{The intruding angles distribution with respect to the ownship~\cite{kochenderfer2009airspace}.}
    \label{fig:encounter}
\end{figure}

==> atms2019_li/sections/3_airspace_density.tex <==
% \section{Airspace Traffic Density} \label{sec:density}
% This section outlines the statistical measures necessary for understanding the dense airspace. 
% We first summarize the metrics typically used to quantify CAS, and then propose a set of metrics that are more appropriate for the dense airspace. 
% We conclude the section with a quantitative definition of the dense airspace.
% The focus of this work is on free flight operations with a horizontal resolution CAS. 
% For cases where airspace structure or other measures of enforcing safety exist other metrics may be more appropriate. 
% The goal of this work is to study the capabilities of CAS individually and save an airspace managed by a mixture of safety-enforcing measures for future work. 

% \subsection{Traditional Metrics for Collision Avoidance}

% The conventional metrics for used to analyze CAS performance are safety and efficiency.
% Safety is typically defined as the rate of NMACs per flight hour. 
% % TODO (max): just say withing some predefined distance of each other?
% In this work we define an NMAC to occur when two aircraft come within 150 meters of each other.
% There are a number of ways to define efficiency, with the most common being the ratio of the flown route length a vehicle took to its destination over the nominal route length .
% We adopt that definition in this work. 

% Throughput has also been recently identified as a relevant metric for CAS evaluation~\cite{bulusu2018throughput}.
% It attempts to measure vehicle flux through an airspace volume per time interval.
% While it is an important metric to consider when analyzing an airspace volume with fixed entry and exit points, it is not appropriate for an airspace with unrestricted take-off and landing areas with vehicles operating in free-flight. 


% \subsection{Metrics for the Dense Airspace}

% A number of metrics have been identified and analyzed to quantify dynamic density in the context of dynamic airspace configuration for the Next Generation Air Transportation System
% (NextGen)~\cite{klein2009simplified, kopardekar2007airspace}.
% % TODO (max): this is too strong here - something about these metrics not capturing the quantities of interest when vehicles are autonomous 
% These metrics aim to analyze the workload capacities of air traffic controllers responsible for the airspace, and may not be relevant in the discussion of a fully autonomous sky. 
% To analyze the dense airspace of fully autonomous vehicles, we make the following observations: traditional metrics fail to capture high-level structural properties of an autonomous airspace, CAS may have a non-trivial impact on the macroscopic properties of the airspace, and the performance of a CAS is more impacted by the difficulty of resolving an encounter rather than the total number of vehicles in an airspace. 

% One way to capture the average decision complexity burden on a CAS in a given airspace is to consider the number of intruder aircraft managed by a collision avoidance system~\cite{golding2018meterics}.
% We extend this notion to a distribution over the average number of intruders in all encounters within the airspace.
% This metric called the encounter distribution, provides a general notion of CAS effectiveness in the airspace, as encounters with more intruders will have a higher likelihood of occurring in a dense airspace and will have a higher likelihood of an NMAC.
% By computing total variation divergence between the encounter distribution for an airspace without an active CAS and one with an active CAS, we can quantify how a CAS changes the encounter structure of an airspace. 
% Namely, given an encounter distribution for an airspace with no active CAS, $P_\text{No}$, and encounter distribution for an airspace with an active CAS, $P_\text{CAS}$, the impact of the active CAS on the airspace is
% \begin{equation}
%     D_\text{TV}(P_\text{No} \parallel P_\text{CAS}) = \frac{1}{2} \sum_{x \in \Omega} |P_\text{No}(x) - P_\text{CAS}(x)|,
% \end{equation}
% where $\Omega$ is the support of the encounter distribution. Lastly, we define a dense airspace with regards to the encounter distribution by making the observation that a CAS will be less effective when it is attempting to resolve a conflict with more than one intruder.
% Formally, we mean that the expectation of a multi-threat encounter is above some threshold value $\lambda$, $\mathbb{E}[N_\text{intruder} > 1] \geq \lambda$, where $N_\text{intruder}$ is the number of intruders in an encounter. 

% % TODO (MAX): add a table of all the metrics here? 

% % We extend the notion of average number of aircraft in the vicinity of the ownship (cite Richar) to address these observations by considering what the distribution over the number of aircraft in an encounter looks like in the whole airspace. 
% % This metric provides a general notion of CAS effectiveness in the airspace, as we expect encounters with more aircraft to have a higher likelihood of an NMAC.
% % We developp the metric further by considering the KL Divergence between the encounter distribution of an airspace without an active CAS on board vehicles and an airspace with an active CAS.
% % 

% % We aim to do the same thing for a CAS by considering a simple concept. A dense airspace would be one that is difficult for a CAS to be perfromant in.  
% % The number of aircraft in an encounter sets a fairly hard limit on the performance of a CAS. We expect the quality of the CAS performance to degreade significantly with increasing number of aircraft. 
% % In Richards work - looks at tbe number of aircraft near 


% % conflict based definition
% %We consider an airspace to be dense when the majority of the conflicts include more than two vehicles. 
% %Formally we say that an airspace is dense if $P(N_{conf} > 1) > 0.5$.
% % Quantitative definition - consider an airspace to be dense when the majority of the conflicts include more than two vehicles. 

% % Dense airspace metrics: add encounter distributions and KL divergence -> measure how CAS changes airspace structure in free flight, average closing time, policy compactness + v_closing/v_cruise 

% % Focus on free flight scenarios. If airspace structure exists, other metrics would be more appropriate such as throughput. 
% % The goal is to capture relevant properties of the dense airspace that are important in CAS design.  
% %For CAS in the ultra-dense airspace, there are two unconventional points: 1. the aircraft of interest are UAVs which typically have small sizes, agile dynamics and quick responses; 2. airspace traffic density is so high that conventional CAS cannot operate properly.

% %The conventional metrics of defining the airspace traffic density include:
% %\begin{itemize}
% %    \item \textit{Spatial traffic density}~\cite{weinert2013uncorrelated}: number of aircraft per unit airspace volume or area;
% %    \item \textit{Encounter density}~\cite{kochenderfer2008correlated}: total number of encounters in a given volume or area for a given period of time.
% %\end{itemize}

% %Conventional metrics include the spatial traffic density~\cite{weinert2013uncorrelated} and the encounter density~\cite{kochenderfer2008correlated}. They are widely used for conventional aircraft. However, they are not universally suitable for airspace consisting of UAVs, VTOL aircraft in low altitude and the notion of the ultra-dense airspace. \citeauthor{bulusu2018throughput} proposed the throughput-based, safety-based and efficiency-based metrics for estimating the airspace capacity~\cite{bulusu2018throughput}. These capacity metrics can also be used for describing the airspace traffic density. Similar to these metrics, we introduce several new quantitative metrics from the perspectives of flight safety and mission efficiency that are able to take the dynamics characteristics of aircraft and the performance of on-board CAS into consideration. 



% %% MAX: the goal of this section is to introduce existing metrics AND to propose a method for quantifying high airspace density

% % Sheng: plots of cross over?
% % Sheng: high density = high likelihood (say, > 50%) of encountering over one intruder before resolving the existing conflict. 

% % MAX: one metric to consider is the following:
% % 1 - (1-Pe)^tr 
% % Where Pe = probability of a conflict encounter per time 
% % tr = average time to resolve a conflict 
% % The threshold we previously talked about is:
% %           1 - (1-Pe)^tr > 0.5
% % This means that more than half of the encounters are multi-threat 

% % Mykel: over 10 times the densest airspace in the US

% % Max: I disagree with Mykel. The whole point of this paper is to come up with a method that can explicitly deal with more than one intruder. I think the way to tell the density story is through a metric that can capture that. Which is exactly the one we've been discussing. It's ok to say something like we simulate an airspace that's 10 times as dense as any airspace in the US - but this doesn't mean much from an operational standpoint. Maybe this still means that ACAS X still works. In fact if most of the encounters are two vehicle encounters in the 10x airspace, that airspace is not dense. Instead defining density based on an encounter metric captures a much more fundamental property that helps us determine how to design systems for managing an airspace. If most of our encounters are more than two vehicle encounters we need to do something other than ACAS X, because ACAS X was designed with a single intruder in mind. 

% % Formal def of dense airspace: a significant fraction of aircraft encounters has more than two vehicles 
% % 1 - (1-Pe)^tr 
